On Robustness of Kernel-Based Regularized System Identification

This paper presents a novel feature of the kernel-based system identification method. We prove that the regularized kernel-based approach for the estimation of a finite impulse response is equivalent to a robust least-squares problem with a particular uncertainty set defined in terms of the kernel matrix, and thus, it is called kernel-based uncertainty set. We provide a theoretical foundation for the robustness of the kernel-based approach to input disturbances. Based on robust and regularized least-squares methods, different formulations of system identification are considered, where the kernel-based uncertainty set is employed in some of them. We apply these methods to a case where the input measurements are subject to disturbances. Subsequently, we perform extensive numerical experiments and compare the results to examine the impact of utilizing kernel-based uncertainty sets in the identification procedure. The numerical experiments confirm that the robust least square identification approach with the kernel-based uncertainty set improves the robustness of the estimation to the input disturbances.

==> mystyleproof.tex <==
%% from here-------------------------
\makeatletter
\DeclareRobustCommand{\qed}{%
  \ifmmode % if math mode, assume display: omit penalty etc.
  \else \leavevmode\unskip\penalty9999 \hbox{}\nobreak\hfill
  \fi
  \quad\hbox{\qedsymbol}}
\newcommand{\openbox}{\leavevmode
  \hbox to.77778em{%
  \hfil\vrule
  \vbox to.675em{\hrule width.6em\vfil\hrule}%
  \vrule\hfil}}
\newcommand{\qedsymbol}{\openbox}
\newenvironment{proof}[1][\proofname]{\par
  \normalfont
  \topsep6\p@\@plus6\p@ \trivlist
  \item[\hskip\labelsep\itshape
    #1.]\ignorespaces
}{%
  \qed\endtrivlist
}
\newcommand{\proofname}{Proof}
\makeatother
%% upto here----------------------------

==> sec_04_syscomp.tex <==
\section{Covariance Design: From System Complexity to Hyperparameter Sparsity}\label{sec:CovDesign}
In real-world applications, many systems have simple structures with low complexity. To reveal the complexity of the system,
one can model or closely approximate a system with the following linear fractional expansion of the transfer function
\begin{equation}\label{eqn:G(z)=simple}
\tilde{G}(\vc{q}) = \sum_{i=1}^s \frac{\tc_i}{\vc{q}-w_i},\quad \tc_i\ne 0,
\end{equation}
where $s$ corresponds to the McMillan degree of the system and assumed to be small.
Motivated by this formulation, for any $w\in\Dbb$, define the {\em atomic transfer function} $\Gw{}$, as the following stable first-order transfer function \citep{shah2012linear} 
\begin{equation}\label{eqn:Gw}
\Gw{}(\vc{q}) = \frac{\alpha_w}{\vc{q}-w},
\end{equation}
where $\alpha_w$ is a positive scalar normalizing a given system norm of $\Gw{}$. In this paper, in line with \citep{shah2012linear}, $\Gw{}$ is normalized with respect to the Hankel nuclear norm with $\alpha_w=1-|w|^2$.
Correspondingly, define the {\em atomic impulse response} $\gw{}$ as the finite impulse response of $\Gw{}$ given by 
\begin{equation}\label{eqn:gw}
\gw{}:= \alpha_w [1, w,\ldots,w^{\nFIR-1}]^\tr \in \Cbb^{\nFIR},
\end{equation} 
and the {\em atomic covariance matrix}
\begin{equation}\label{eqn:Sw}
    \Sw{} = \gw{}\left({\gw{}}\right)^\Hr\in \Hbb^{\nFIR}_+.
\end{equation}
    As proved in \citep{Chen_2012}, when the underlying system is exactly $\Gw{}(\vc{q})$, the optimal kernel selection is given by $\Sw{}$. %This motivates the selection of $\Sw{}$ as the atomic covariance matrix.

One can easily see that $\tilde{G}(\vc{q})$ given in \eqref{eqn:G(z)=simple} is a linear combination of atomic transfer functions, i.e., $\{\Gw{}\}_{w\in\Dbb}$ spans the space of transfer functions of the form given in \eqref{eqn:G(z)=simple}.

Let $\neta\in\Nbb$ and $\Wcal  = \{w_1,\ldots,w_{\neta}\}\subset \Dbb$ be a set of $\neta$ stable distinct poles. For real-valued systems, it is required that for any $w\in\Wcal$, one has $w^*\in\Wcal$. The following structure of $\mx{S}_{\eta}$ is proposed
\begin{equation}\label{eqn:Seta}
\mx{S}_{\eta} = \sum_{i=1}^{\neta}\eta_i \Sw{i}= \sum_{i=1}^{\neta}\eta_i \gw{i}\left({\gw{i}}\right)^\Hr,
\end{equation}
where $[\eta_1\ \eta_2\ \ldots\  \eta_{\neta}]^\tr\in\Rbb^{\neta}_+$ is denoted by $\eta$. To satisfy the constraint of $\mx{S}_\eta\in\Sbb_+^{\nFIR}$, it is noted that $\Sw{i}=\left(\Sw{j}\right)^*$ for any $w_i = w_j^*$. So, $\eta$ is constrained to satisfy
\begin{equation}\label{eqn:constaint}
\eta_i=\eta_j,\qquad \forall i,j \text{ such that } w_i = w_j^*.
\end{equation}
%\begin{remark}
%	One can easily see that $\rank(\mx{S}_\eta)\le \|\eta\|_0$.
%\end{remark}	
Based on this definition, we have the following theorem which is the theoretical foundation of the method proposed in this paper.
%_________________________________________
\begin{theorem}\label{thm:Srank}
Let $\vc{\hat{g}}$ be a realization sample of the impulse response prior distribution $\Ncal(\zero,\mx{S}_\eta)$, where $\mx{S}_\eta$ satisfies \eqref{eqn:Seta}. 
Then, there exists $\vc{c}=[c_1\ c_2\ \ldots\ c_{\neta}]^\tr\in\Cbb^{\neta}
$ such that the following hold.\\
{\rm i)} 
For any $i,j$ satisfying $w_i = w_j^*$, we have $c_i=c_j^*$.\\
{\rm ii)} 
The sample realization impulse response $\vc{\hat{g}}$ can be decomposed as
$\vc{\hat{g}}= \sum_{i=1}^{\neta}c_i\mathbf{1}_{\{\eta_i\ne 0\}}(\eta)\ \gw{i}
$.\\
%\begin{equation}\label{eqn:geta1}
%\vc{\hat{g}}=\sum_{i=1}^{\neta}\big{(}c_i \mathbf{1}_{\{\eta_i\ne 0\}}(\eta)\big{)} \ \gw{i},
%\end{equation}
{\rm iii)} 
Let $\vc{g}_{\vc{c}}\in\Rbb^{\nFIR}$ be a finite impulse response which corresponds to a transfer function, denoted by $G_{\vc{c}}$ and defined as 
$G_{\vc{c}}(\vc{q})=\sum_{i=1}^{\neta}\big{(}c_i \mathbf{1}_{\{\eta_i\ne 0\}}(\eta)\big{)} \Gw{i}(\vc{q})$.
%\begin{equation}\label{eqn:Geta1}
%G_{\vc{c}}(\vc{q})=\sum_{i=1}^{\neta}\big{(}c_i \mathbf{1}_{\{\eta_i\ne 0\}}(\eta)\big{)} \Gw{i}(\vc{q}),
%\end{equation}
Then, one has $\vc{g} = \vc{g}_{\vc{c}} $.
\end{theorem}
%_________________________________________
%_________________________________________
\begin{corollary}\label{cor:sparsity}
	The poles of $G_{\vc{c}}(\vc{q})$ is a subset of $\{w_i\ |\ i\in \supp(\eta)\}$ and the McMillan degree of $G_{\vc{c}}(\vc{q})$ is less than or equal to $\|\eta\|_0$.
	Therefore, any $\vc{g} \sim \Ncal(\zero,\mx{S}_\eta)$ corresponds to a system with a McMillan degree of at most $\|\eta\|_0$.  
\end{corollary}

According to Theorem \ref{thm:Srank} and Corollary \ref{cor:sparsity}, it can be seen that the desired low-complexity structure of the system is induced by the sparsity of the hyperparameters $\eta$. However, in order to have a favorable estimation of the impulse response, the set $\Wcal$ should be nearly dense in $\Dbb$. Accordingly, it is advantageous to employ a large set of basis covariance matrices.
This suggests performing sparse estimation at the level of hyperparameter tuning, which will be discussed in the next section. Meanwhile, a satisfactory bias-variance trade-off at the level of impulse response estimation is maintained by utilizing the regularized identification method in \eqref{eqn:RegLS}.

\begin{remark}\label{rem:5}
This characteristic differs from the atomic-norm regularization in \citep{shah2012linear}, where $l_1$-norm regularization is directly imposed on the decomposition coefficient vector $\vc{c}$ at the level of impulse response estimation. This direct sparsity regularization adds more regularization to the impulse response estimation. The atomic-norm regularization is known to suffer from high bias as discussed in \citep{Pillonetto_2016}.
\end{remark}


==> sec_05_hypREB.tex <==
\section{Hyperparameter Tuning: an MAP Approach}\label{sec:Hyper}
This section present a MAP approach that imposes additional sparsity regularization for the estimation of the hyperparameters introduced in Section \ref{sec:CovDesign}.

\subsection{MAP Estimation of Hyperparameters}
Define set $\Ical^+$ 
%and $\Wcal^+$ 
as $\Ical^+ = \{i\in \{1,\ldots,n_\eta\}\  | \ \imag{w_i} \ge 0 \}$.
%\begin{equation}
%\begin{split}
%\Ical^+ &= \{i\in \{1,\ldots,n_\eta\}\  | \ \imag{w_i} \ge 0 \}.\\
%%\Wcal^+ &= \{w\in \Wcal\  | \ \imag{w} \ge 0 \}.
%\end{split}
%\end{equation}
According to the structural constraint of $\Seta$ in \eqref{eqn:constaint}, one only needs to estimate $\eta_i$, for $i\in\Ical^+$. The remaining hyperparameters are determined automatically. 
In this section, with an abuse of notation, $\eta$ denotes the vector of independent hyperparameters $(\eta_i)_{i\in\Ical^+}$. Accordingly, $\neta$ is the length of $\eta$.
% Similarly, we denote $\Wcal$ as $\{w_i\in\Wcal\ |\ i\in\Ical^+ \}$.

In order to introduce an MAP estimation approach for $\eta$, the following prior, that promotes the sparsity of the hyperparameters $\eta$, is defined.
Since the entries of $\eta$ are initially (a priori) undiscriminating and independent, the prior of each entry of $\eta$ is selected as an i.i.d. exponential distribution \citep{aravkin2014convex}.  
More precisely, for any $i$, we have $
p(\eta_i) = \lambda\exp(-\lambda \eta_i)\mathbf{1}_{\{\eta_i\ge 0\}}(\eta_i)$,
where $\lambda>0$ is the {\em  rate parameter} of the distribution. The ``hyper-hyperparameter'' $\lambda$ parameterizes the prior on the hyperparameter. In this paper, $\lambda$ is estimated by cross validation. Accordingly, we have
\begin{equation}\label{eqn:p(eta)}
p(\eta) = 
\lambda^{n_\eta}\exp(-\lambda\sum_{i=1}^{n_\eta} \eta_i) \  \mathbf{1}_{\{\eta\in\Rbb_+^{n_\eta}\}}(\eta).
\end{equation}
From \eqref{eqn:gyN(...)}, we know that 
\begin{equation}\label{eqn:p(y|eta)}
\mx{y}|\eta \sim \Ncal(\zero, \Phi\mx{S}_{\eta}\Phi^\tr + \sigma_w^2\eye).
\end{equation}
By Bayes' rule, one can estimate the vector of hyperparameters by MAP estimation as follows.
\begin{equation}\label{eqn:etaMAP}
\etaMAP 
%=  \argmax_{\eta\in\Rbb^{n_\eta}}\ p(\eta|\vc{y}) 
=  \argmax_{\eta\in\Rbb^{n_\eta}}\ p(\vc{y}|\eta)p(\eta),
\end{equation} 
where the denominator in the Bayes fraction $p(\vc{y})$ is removed due to being independent of $\eta$.
From \eqref{eqn:p(eta)}, \eqref{eqn:p(y|eta)}, \eqref{eqn:etaMAP}, and the monotonicity of the logarithm function, one can see that
%\begin{equation}\label{eqn:etaMAP2}
%\begin{array}{cccl}
%\etaMAP & = & \argminOp_{\eta\in\Rbb_+^{n_\eta}} &
%\frac{1}{2}\vc{y}^\tr\Sigma^{-1}\vc{y} 
%+
%\frac{1}{2}\log\!\det\Sigma + \lambda \sum_{i=1}^{n_\eta}\eta_i,
%\\& & {\text{s.t.}} &\Sigma =\Phi\mx{S}_{\eta}\Phi^\tr + \sigma_w^2\eye.
%\end{array}\!\!
%\end{equation}
\begin{equation}\label{eqn:etaMAP2}
\etaMAP\!\!\!=\!\argmin_{\eta\in\Rbb_+^{n_\eta}}\ \! 
\frac{1}{2}\vc{y}^\tr\!\Sigma_\eta^{-1}\vc{y} 
\!+\!
\frac{1}{2}\log\!\det\Sigma_\eta 
\!+\! 
\lambda \sum_{i=1}^{n_\eta}\eta_i,
\!\!
\end{equation}
where $\Sigma_\eta =\Phi\mx{S}_{\eta}\Phi^\tr + \sigma_w^2\eye$.

The following proposition provides the theoretical basis for solving the hyper-estimation problem \eqref{eqn:etaMAP2} efficiently.
\begin{proposition}\label{prp:dcp}
	Optimization problem \eqref{eqn:etaMAP2} can be expressed as a DCP problem. 
\end{proposition}
\begin{proof}
%%Note that $\Seta$ depends on $\eta$ linearly. Therefore, any convex function of $\Seta$ is convex with respect to $\eta$ as well, if $\Seta$ is in the domain of the function. 
%%Since $\sigma_w^2>0$, we have that $\Sigma_\eta\in \Sbb_{++}^{n_\eta}$, for any  $\eta \in \Rbb_+^{n_\eta}$.
%%For a given $\vc{y}$, define functions $f,h:\Sbb_{++}^{n}\to \Rbb$ as $f(\Sigma) = \frac{1}{2}\vc{y}^\tr\Sigma^{-1}\vc{y}$ and $h(\Sigma) = -\frac{1}{2}\log\!\det\Sigma$.
%%%\begin{equation}
%%%\begin{array}{rll}
%%%f(\Sigma) = \frac{1}{2}\vc{y}^\tr\Sigma^{-1}\vc{y},  
%%%%&\quad
%%%%\forall \Sigma \in \Sbb_{++}^{n},
%%%h(\Sigma) = -\frac{1}{2}\log\!\det\Sigma.
%%%%&\quad
%%%%\forall \Sigma \in \Sbb_{++}^{n}.
%%%\end{array}
%%%\end{equation}
%%These two functions are convex on their domain \citep{boyd2004convex}. 
%%Accordingly, $f(\Sigma_\eta)$ and $g(\Sigma_\eta)$ are convex functions with respect to $\eta$.
%%The final term $\lambda \sum_{i=1}^{n_\eta}\eta_i$ is linear with respect to $\eta$ and therefore convex.
Let $F,H:\Rbb_+^{n_\eta}\to \Rbb$ be defined as
\begin{equation}\label{eqn:F_and_H}
F(\eta)  = \frac{1}{2}\vc{y}^\tr\Sigma_\eta^{-1}\vc{y} + \lambda \sum_{i=1}^{n_\eta}\eta_i,
H(\eta)  = -\frac{1}{2}\log\!\det\Sigma_\eta. 
\end{equation}
One can easily see that $F$ and $H$ are convex functions and the objective function in \eqref{eqn:etaMAP2} is $F(\eta)-H(\eta)$. This concludes the proof.
\end{proof}	
According to Proposition \ref{prp:dcp}, one can obtain a stationary point of the optimization problem \eqref{eqn:etaMAP2} efficiently.
In this regard, the problem can be solved by an appropriate solver designed for disciplined programming of DCP problems \citep{shen2016disciplined}, or a suitable algorithm for solving this type of optimization problem, e.g. \cite{yuille2002concave}.
Here, the latter approach is applied which is essentially a majorization minimization (MM) algorithm and solves the problem using a sequential convex programming scheme.
In detail, a {\em majorization} function $J:\Rbb_+^{n_\eta}\times\Rbb_+^{n_\eta}\to \Rbb$ can be defined, if we have
\begin{align}
J(\eta,\eta)   &= F(\eta)- H(\eta), \qquad \forall \eta\in\Rbb_+^{n_\eta},\label{eqn:mmcon}\\
J(\eta,\gamma) &\ge F(\eta)- H(\eta),\qquad \forall \eta,\gamma\in\Rbb_+^{n_\eta}.\label{eqn:mmcon2}
\end{align}
Following this, the method solves the problem iteratively using the following procedure
\begin{equation}
\eta^{(k+1)} = \argmin_{\eta\in\Rbb_+^{n_\eta}}J(\eta,\eta^{(k)}).
\end{equation} 
Here, the majorization function is defined by replacing $H(\eta)$ with its linearization at $\gamma$ in the objective function. Then, constraints \eqref{eqn:mmcon} and \eqref{eqn:mmcon2} are satisfied due to the convexity of $H(\eta)$. More precisely, we have
\begin{equation}\label{eqn:J}
J(\eta,\gamma):= F(\eta) - H(\gamma)- \nabla_{\gamma}H(\gamma)^\tr(\eta-\gamma),
\end{equation} 
where
\begin{equation}\label{eqn:grad}
\nabla_{\eta_i}H(\eta)=-\frac{1}{2}\text{tr}\left(\Sigma_\eta^{-1}\Phi\Sw{i}\Phi^\tr\right).
\end{equation}
Note that the term $H(\gamma)$ does not depend on the optimization variable $\eta$ and can thus be removed.

The hyperparameter tuning procedure, by solving the MAP estimate \eqref{eqn:etaMAP2} with the MM algorithm, is summarized in Algorithm \ref{alg:dcp}. Then, the FIR model  is identified by \eqref{eqn:gmap} with $\mx{S} = \mx{S}_{\etaMAP}$.
%__________________________________________________
\begin{algorithm}[t]
	\caption{MAP-based hyperparameter tuning}\label{alg:dcp}
	\begin{algorithmic}[1]
		\State \textbf{Input:} $\vc{y}$,$\Phi$,$\Wcal$
		\State Calculate $\mx{S}^{(w)}$, for $w\in \Wcal$ (see \eqref{eqn:Sw} and \eqref{eqn:gw}).
		\State $k\leftarrow 0$, initialize $\eta^{(0)}$.
		\While{stopping condition is not met}
		%\Statex
		%\Comment{$k_{\text{final}}$ is the DDPC final time horizon}
		\State Calculate $\nabla_{\eta^{(k)}}H(\eta^{(k)})$ (see \eqref{eqn:grad}) and 
		\State From \eqref{eqn:F_and_H} and \eqref{eqn:J}, set the function $J$ as
		$$J(\eta,\eta^{(k)}) = F(\eta) - \nabla_{\eta^{(k)}}H(\eta^{(k)})(\eta-\eta^{(k)}).$$
		\State Solve convex optimization problem
		$$\eta^{(k+1)} = \argmin_{\eta\in\Rbb_+^{n_\eta}}
		J(\eta,\eta^{(k)}).$$
		\State $k\leftarrow k+1$.
		\EndWhile\label{DCP_loop}
		\State \textbf{end} 
		\State \textbf{Output:} $\etaMAP = \eta^{(k)}$
	\end{algorithmic}
\end{algorithm}
%____________________________________________
\subsection{Empirical Bayes and Regularized Empirical Bayes}\label{sec:eb}
In the empirical Bayes method \citep{chen2014system}, the hyperparameters are estimated by maximizing the marginal likelihood, 
%so that the probability of observing $\vc{y}$ is maximized, 
i.e., $\etaEB =  \argmax_{\eta\in\Rbb^{n_\eta}_+}\ p(\vc{y}|\eta)$.
%\begin{equation}\label{eqn:etaEB}
%\etaEB 
%=  \argmax_{\eta\in\Rbb^{n_\eta}_+}\ p(\vc{y}|\eta).
%\end{equation}
Note that there is an implicit prior on the hyperparameters, which is $\eta\in\Rbb^{n_\eta}_+$. The method is essentially a ML approach which is also known as {\em type-II maximum likelihood} \citep{good1965estimation}.
The empirical Bayes method performs well when the number of hyperparameters is not large and the data set is not significantly small or noisy. 
However, as discussed in Section \ref{sec:CovDesign}, here a considerably large number of hyperparameters are to be estimated . In this situation, the solution of the empirical Bayes method is prone to high variance. Consequently, it is preferable to employ the MAP approach, especially when the prior knowledge on the sparsity of the hyperparameters is available. 

From \eqref{eqn:p(y|eta)}, one can see that
\begin{equation}\label{eqn:etaEB2}
\etaEB = \argmin_{\eta\in\Rbb_+^{n_\eta}} \
\frac{1}{2}\vc{y}^\tr\Sigma_\eta^{-1}\vc{y} 
+
\frac{1}{2}\log\!\det\Sigma_\eta.
\!\!
\end{equation}
The difference between \eqref{eqn:etaMAP2} and \eqref{eqn:etaEB2} is a single term in the objective function, i.e., $\lambda \sum_{i=1}^{n_\eta}\eta_i$, which comes from the sparse prior.
In fact, this term performs a regularization on the estimation of the hyperparameters and subsequently improves the bias-variance trade-off. 
Therefore, one can alternatively call $\etaMAP$ as the solution of the {\em regularized empirical Bayes} estimation and denote it by $\etaREB$.

One should note that the empirical Bayes method may also induce sparsity in the estimation of the hyperparameters in a high-dimensional setting.
This is due to the implicit prior of non-negative $\eta$. However, the induced sparsity is governed by the data rather than assumed prior, % without an MAP nature, 
and thus can be noise-dependent. 
In the method proposed here, the sparsity is governed by the prior knowledge (low-complexity in this case) of the system. 
As a consequence, the estimation encodes  more system-dependent features comparing to the empirical Bayes method, which makes it more robust with respect to measurement noise.
Here, the sparsity of the estimator is controlled by the rate parameter $\lambda$. Meanwhile, one can still obtain the empirical Bayes estimate by setting $\lambda=0$.


==> sec_06_sim.tex <==
\section{Numerical Results}

In this section, the proposed sparse hyperparameter tuning method is compared to other existing regularization formulation with the atomic structure. For the baseline performance, the least squares method without regularization and the well-known first-order stable spline kernel, also known as the TC kernel, introduced in \citep{Chen_2012} are also compared. Note that these two methods do not estimate a low-complexity model.
Specifically, the following five identification schemes are compared. The least squares method (\textit{LS}) corresponds to the estimate $\gML$ in \eqref{eqn:ML}. 
The system is also identified with a TC kernel (\textit{TCK}) regularization. The hyperparameters are selected by the empirical Bayes method with a non-convex optimization. This is also the defaulted identification method used in the \textsc{Matlab} command \texttt{impulseest}.
The atomic-norm method (\textit{Atom}) applies the atomic-norm regularization proposed in \citep{shah2012linear}. \textit{Atom} applies a set of atomic transfer function characterized by the poles $w_i=r\cdot e^{j\phi}$, where $\phi=[0:\pi/15:\pi]$ in the \textsc{Matlab} notation. The magnitude $r$ is in a 15-point logspace grid of base $10^6$ between 0.8 and 1 to obtain a denser grid near $r=1$. The empirical Bayes method (\textit{EB}) uses the hyperparameter estimation scheme \eqref{eqn:etaEB2} introduced in \citep{chen2014system} without explicitly exploiting the sparse kernel structure. The regularized empirical Bayes method (\textit{REB}) refers to the method proposed in this paper (Algorithm \ref{alg:dcp}). Both \textit{EB} and \textit{REB} regularize the problem with the first-order kernel set $\Scal$ paramerized by \eqref{eqn:Seta} with the same set of poles as \textit{Atom}. This gives a total of $\neta=240$ kernels. 

To highlight the characteristics of the bias-variance trade-off in these methods, numerical simulations are conducted on a benchmark system under i.i.d Gaussian noise of three different levels ($\sigma^2=0.1,0.01,0.001$) with 150 different noise realizations each. The transfer function of the chosen fourth-order discrete-time LTI system is
\begin{equation}
    G(z) = \frac{z^3+0.5z^2}{z^4-2.2z^3+2.42z^2-1.87z+0.7225}
\end{equation}
which is one of the benchmark systems tested in \citep{pillonetto2010new}. The input to the system is Gaussian with $u(t)\sim \Ncal(0,1)$. The length of the identification data is $\nD=150$ and the order of the FIR model is $\nFIR=50$. For \textit{EB} and \textit{REB}, the noise variance $\sigma^2$ is estimated from the variance of the residuals in \textit{LS}. For \textit{Atom} and \textit{REB}, the weighting of the $l_1$-norm regularization and the rate parameter $\lambda$ are cross-validated over a five-point grid of \texttt{logspace(0,4,5)} and \texttt{logspace(-1,1,5)} in the \textsc{Matlab} notation, respectively. The DCP optimization problem in \textit{REB} is solved by a fixed number of five iterations.

First, the fitting performance of the five methods are compared in Fig.~\ref{fig:mc} using box plots. The fits of the estimates are defined as
\begin{equation}
W=100\times \left(1-\left[\frac{\sum_{i=1}^{n_g}(g_i-\hat{g}_i)^2}{\sum_{i=1}^{n_g}(g_i-\bar{g})^2}\right]^{1/2}\right),
\end{equation}
where $g_i$ are the true impulse response coefficients, $\hat{g}_i$ are the estimated coefficients, and $\bar{g}$ is the mean of the true coefficients. %This measure is equivalent to the \texttt{compare} function in the System Identification Toolbox.

\begin{figure}[htbp]
\centering
%\subfloat[$\sigma^2=0.1$]{\includegraphics[width=3.45in]{fig/sig1e-1.eps}}\\
\subfloat[$\sigma^2=0.01$]{\includegraphics[width=1.725in]{fig/sig1e-2.eps}}
\subfloat[$\sigma^2=0.001$]{\includegraphics[width=1.725in]{fig/sig1e-3.eps}}
\caption{Comparison of fitting performance under different noise levels. The last three methods estimate a low-complexity model with atomic structure.}
\label{fig:mc}
\end{figure}


As can be seen from Fig.~\ref{fig:mc}, \textit{REB} achieves the best fitting performance at all three noise levels. Compared to \textit{REB}, the performance of \textit{EB} is poor under the high noise level, whereas \textit{Atom} and \textit{TCK} perform worse under the low noise level. In all three cases, \textit{LS} fails to achieve a good performance without regularization.
Furthermore, the bias and the variance of the estimates are calculated in Table~\ref{tbl:mc}. It can be seen, as discussed in \citep{pillonetto2014kernel}, that the bias-variance trade-off is controlled by the amount of regularization imposed. The mean square error (MSE) of \textit{LS} is dominated by the variance since no regularization is imposed. Note that there is an inherent bias induced by the impulse response truncation. \textit{Atom}, conversely, induces the highest amount of bias with $l_1$-norm regularization. The proposed method \textit{REB} imposes more regularization than \textit{EB} with an additional sparsity regularization in hyperparameter tuning, but less regularization compared to the direct sparsity regularization on the impulse response estimation as in \textit{Atom}. This characteristic leads to an appropriate balance in terms of the bias-variance trade-off as can be seen from the MSE values. This result agrees with the discussion in Remark~\ref{rem:5} and Section~\ref{sec:eb}.

\begin{table}[htbp]
\renewcommand{\arraystretch}{1.2}
\caption{Bias-variance trade-off}
\label{tbl:mc}
\centerline{
\begin{tabular}{ccccccc}
\hline\hline
&\textbf{LS}& \textbf{TCK}& \textbf{Atom} & \textbf{EB} & \textbf{REB} \\ \hline 
\textbf{$\sigma^2=0.01$}&&&&& \\
\textbf{$\text{Bias}^2\ [\times 10^{-4}]$} & 1.6  & 8.5  & 11.2 & 5.6  & 8.4  \\
\textbf{$\text{Var}\ [\times 10^{-4}]$}    & 61.0 & 23.6 & 17.1 & 20.8 & 12.3 \\ 
\textbf{$\text{MSE}\ [\times 10^{-4}]$}    & 62.6 & 32.1 & 28.3 & 26.4 & \textbf{20.8} \\ \hline
\textbf{$\sigma^2=0.001$}&&&&& \\
\textbf{$\text{Bias}^2\ [\times 10^{-4}]$} & 0.15 & 0.96 & 1.24 & 0.37 & 0.68 \\
\textbf{$\text{Var}\ [\times 10^{-4}]$}    & 6.23 & 3.79 & 2.97 & 2.98 & 2.52 \\
\textbf{$\text{MSE}\ [\times 10^{-4}]$}    & 6.38 & 4.75 & 4.21 & 3.35 & \textbf{3.20} \\ \hline\hline
\end{tabular}
}
\end{table}
